Amplitude-Aware Lossy Compression for Quantum Circuit Simulation

Classical simulation of quantum circuits is crucial for evaluating and validating the design of new quantum algorithms. However, the number of quantum state amplitudes increases exponentially with the number of qubits, leading to the exponential growth of the memory requirement for the simulations. In this paper, we present a new data reduction technique to reduce the memory requirement of quantum circuit simulations. We apply our amplitude-aware lossy compression technique to the quantum state amplitude vector to trade the computation time and fidelity for memory space. The experimental results show that our simulator only needs 1/16 of the original memory requirement to simulate Quantum Fourier Transform circuits with 99.95% fidelity. The reduction amount of memory requirement suggests that we could increase 4 qubits in the quantum circuit simulation comparing to the simulation without our technique. Additionally, for some specific circuits, like Grover's search, we could increase the simulation size by 18 qubits.

==> conclusion.tex <==
\section{Conclusion}
The simulation of quantum circuits is an important topic to advance the quantum computing research.
The capability of the simulation is limited by the memory capacity of the classical computer.
We present a full state quantum circuits simulation technique to simulate more qubits than previously reported by using lossy data compression.
Since we know most of the quantum state amplitudes in different quantum algorithms are close to 0, similar to the benchmarks we showed in this paper, we expect our technique can be widely used for simulating various quantum algorithms.
Our approach compress the state vector to reduce the memory requirement, so the we can simulate a larger quantum system with the same memory capacity.
Lossy data compression introduces errors to the simulation.
This error could potentially model the presence of the physical noise in the quantum circuits.
In the future work, we plan to run 56-qubit simulation on Theta, analyze the effect of compression errors and relationships to real physical noise, integrate our technique with other approximate simulation techniques, and evaluate different compression algorithms for quantum state amplitudes.




